Improved Learning-augmented Algorithms for k-means and k-medians Clustering

We consider the problem of clustering in the learning-augmented setting, where we are given a data set in $d$-dimensional Euclidean space, and a label for each data point given by an oracle indicating what subsets of points should be clustered together. This setting captures situations where we have access to some auxiliary information about the data set relevant for our clustering objective, for instance the labels output by a neural network. Following prior work, we assume that there are at most an $\alpha \in (0,c)$ for some $c<1$ fraction of false positives and false negatives in each predicted cluster, in the absence of which the labels would attain the optimal clustering cost $\mathrm{OPT}$. For a dataset of size $m$, we propose a deterministic $k$-means algorithm that produces centers with improved bound on clustering cost compared to the previous randomized algorithm while preserving the $O( d m \log m)$ runtime. Furthermore, our algorithm works even when the predictions are not very accurate, i.e. our bound holds for $\alpha$ up to $1/2$, an improvement over $\alpha$ being at most $1/7$ in the previous work. For the $k$-medians problem we improve upon prior work by achieving a biquadratic improvement in the dependence of the approximation factor on the accuracy parameter $\alpha$ to get a cost of $(1+O(\alpha))\mathrm{OPT}$, while requiring essentially just $O(md \log^3 m/\alpha)$ runtime.

==> old.tex <==
\section{Notations}
Given a set of points $X \subseteq \mathbb{R}$ of size $m$, we have the following disjoint partitions based on an optimal $k$-means solution,  $X_1^\star,\ldots, X_k^\star$, and $\cup_{i=1}^k X_i^\star = X$. We also have the partition based on a classifier, $X_1,\ldots, X_k$, and $\cup_{i=1}^k X_i = X$. Let $P_i = X_i \cap X_i^\star$, and $\err \in (0,1) $, we assume $\frac{|P_i|}{|X_i|} \geq 1-\err$ and $\frac{|P_i|}{|X_i^\star|} \geq 1-\err$. Let $X_{i,j} , X_{i,j}^\star$, $P_{i,j}$  be the dimension $j$ of partition $i$ from the classifier, the optimal $k$-means solution, and  $P$ respectively. Let $m_i = |X_i|, m^\star_i = |X^\star_i|$. Denote $\diam{S}$ the diameter of the set $S$. 
\section{Algorithm}
Let $\bb \in (0,1)$. For each $i,j$, let $I_{i,j}$ be the intersection of the smallest interval containing $m_i(1-\err - \bb)$ points with $X_{i,j}$. For $i=1\ldots,k$, let $C'_i = \{\overline{I_{i,1}},\ldots,\overline{I_{i,d}}\}$. Return $C'_1,\ldots, C'_k$.

\section{Analysis}
\begin{lemma}
\label{fig:outliers}
%There are $\frac{\bb m}{2}$ points in $P_{i,j}$ that are at least $\frac{|I_{i,j}|}{2}$ away from $\overline{P_{i,j}}$.
For all $i \in [k], j \in [d]$, there exists a set $Q_{i,j} \subseteq P_{i,j}$ such that $|Q_{i,j}| \geq \bb m_i$ and $|q - \overline{P_{i,j}}| \geq \frac{\diam{I_{i,j}}}{2}$ for all $q \in Q_{i,j}$.
\end{lemma}
\begin{proof}
For all $i \in [k], j \in [d]$, note that the $\frac{\diam{I_{i,j}}}{2}$-ball of $\overline{P_{i,j}}$ contains at most $m_i(1-\alpha - \bb)$ points in $P_{i,j}$. Since $|P_i| \geq m_i(1-\alpha)$, there must be at least $\bb m_i$ points in $P_{i,j}$ that lie outside of the ball. 
\end{proof}

% \begin{lemma}
% \label{fig:outliers}
% %There are $\frac{\bb m}{2}$ points in $P_{i,j}$ that are at least $\frac{|I_{i,j}|}{2}$ away from $\overline{P_{i,j}}$.
% For all $i \in [k], j \in [d]$, there exists a set $Q_{i,j} \subseteq P_{i,j}$ such that $|Q_{i,j}| \geq \frac{\bb m_i}{2}$ and $|q - \overline{P_{i,j}}| \geq |I_{i,j}|$ for all $q \in Q_{i,j}$.
% \end{lemma}
% \begin{proof}
% Recall that $|P_{i}| \geq (1-\alpha) m_i $.  Suppose there are $\frac{(1-\alpha) m_i}{2}$ points in $P_{i,j}$ at most $\overline{P_{i,j}}$. Consider the sorted array of $P_{i,j}: \{ p_1,\ldots p_{|P_i|}\}$, and the interval  $I_{i,j}' = [p_{\frac{\beta m_i }{2}}, \overline{P_{i,j}}]$. Note that $I_{i,j}'$ contains at least  $\frac{m_i(1-\err - \bb)}{2}$ points in $X_{i,j}$. This means $ \overline{P_{i,j}} - p_{i} \geq |I_{i,j}|$ for $i \leq  p_{\frac{\beta m_i}{2}}$.

% The other case is there are at least  $\frac{(1-\alpha) m_i}{2}$ points in $P_{i,j}$ at least $\overline{P_{i,j}}$, and the argument follows similarly.

% \end{proof}
From lemma~\ref{fig:outliers}, we derive a lower bound on $\cost{X_{i,j}^\star}{X_{i,j}^\star}  $.

\begin{lemma}
For all $i \in [k], j \in [d]$, $ \cost{X_{i,j}^\star}{X_{i,j}^\star}  \geq \frac{\diam{I_{i,j}}^2 \bb m_i}{4}  $.
\end{lemma}
\begin{proof}
The lemma follows by the fact that \begin{align*}
    \cost{P_{i,j}}{P_{i,j}} \leq  \cost{P_{i,j}}{X^\star_{i,j}} \leq \cost{X^\star_{i,j}}{X^\star_{i,j}} 
\end{align*}
\end{proof}
We have the following standard lemma. 

\begin{lemma}
\label{lemma:lambda_mean}
Let $J_1, J_2 \subseteq \mathbb{R} $ be disjoint sets  such that $|J_1| \geq (1-\lambda) n$ and $|J_2| \leq \lambda n$ where $n = | J_1 \cup J_2| = |J| $. Then $|\overline{J_1} - \overline{J}|^2 \leq \frac{\lambda}{(1-\lambda) n} \cost{J}{J}$.
\end{lemma}
\begin{proof}
 We know $|J_1| = (1-x) n, |J_2| = xn$ for $x \leq \lambda$. Then $\overline{J} = (1-x) \overline{J_1} + x \overline{J_2}$. We thus have 
 \begin{align*}
    & | \overline{J} - \overline{J_1}| = x |\overline{J_2} - \overline{J_1}|     \\  & | \overline{J} - \overline{J_2}| = (1-x) |\overline{J_2} - \overline{J_1}| \\ 
    &\implies  | \overline{J} - \overline{J_2}| = \frac{1-x}{x} |\overline{J} - \overline{J_1}| \numberthis{} \label{distJ_J2}  .
 \end{align*}
 By convexity,  
 \begin{align*}
     \cost{J}{J} = \cost{J_1}{J_1} +  \cost{J_2}{J_1} & \geq (1- x) n |\overline{J} - \overline{J_1}|^2 + x n   |\overline{J} - \overline{J_2}|^2 \\
     & = (1- x) n |\overline{J} - \overline{J_1}|^2 + \frac{(1-x)^2 n}{x}   |\overline{J} - \overline{J_1}|^2 \\ 
     & = \frac{(1-x)n }{x} |\overline{J} - \overline{J_1}|^2 \\
     & \geq \frac{(1-\lambda)n }{\lambda} |\overline{J} - \overline{J_1}|^2.
 \end{align*}
\end{proof}
% \begin{proof}
% WLOG $\overline{J} = 0$.  Suppose $|J_1| = (1-x) n, |J_2| = xn$ for $x \leq \lambda$. We thus have $\overline{J_2} = - \frac{1-x}{x}  \overline{J_1}$. If $x \leq 0.5$, we lower bound $\cost{J_2}{J}$ by convexity  
% \begin{align*}
%     \cost{J_2}{J} \geq \frac{1}{|J_2|} \left(\sum_{j \in J_2} j\right)^2  
%                   =  \frac{|J_2|^2}{|J_2|} \overline{J_2}^2  
%                   = |J_2| \cdot \frac{(1-x)^2}{x^2} \cdot \overline{J_1}^2  
%                   \geq |J_2| \cdot \frac{1}{4x^2} \cdot \overline{J_1}^2 
%                  & = \frac{n}{4x} \cdot \overline{J_1}^2 \\ 
%                  & = \frac{n}{4x} \cdot | \overline{J_1} - \overline{J}| ^2. 
% \end{align*}
% Thus,
% \begin{align*}
%     \cost{J}{J} \geq \cost{J_2}{J} \geq   \frac{n}{4x} \cdot | \overline{J_1} - \overline{J}| ^2 \geq \frac{n}{4\lambda} \cdot | \overline{J_1} - \overline{J}| ^2  
% \end{align*}

% If $x \geq 0.5$,  we lower bound $\cost{J_1}{J}$ by convexity
% \begin{align*}
%      \cost{J_1}{J} \geq \frac{1}{|J_1|} \left(\sum_{j \in J_1} j\right)^2  
%                   =  \frac{|J_1|^2}{|J_1|} \overline{J_1}^2 = |J_1|\cdot \frac{x^2}{(1-x)^2} \cdot  \overline{J_2}^2  \geq \frac{n}{4(1-x)} \cdot \overline{J_2}^2  & = \frac{n(1-x)}{4x^2} \cdot \overline{J_1}^2 \\ & = \frac{n(1-x)}{4x^2} \cdot |\overline{J} - \overline{J_1}|^2 .
% \end{align*}
% Thus,
% \begin{align*}
%     \cost{J}{J} \geq \cost{J_1}{J} \geq   \frac{n(1-x)}{4x^2} \cdot |\overline{J} - \overline{J_1}|^2 \geq  \frac{n(1-\lambda)}{4\lambda^2} \cdot |\overline{J} - \overline{J_1}|^2.
% \end{align*}
%  Thus, \begin{align*}
%      |\overline{J} - \overline{J_1}|^2 \leq 4 \max\left(\frac{\lambda^2}{1-\lambda}, \lambda\right) \frac{\cost{J}{J}}{n} \leq \frac{4\lambda}{(1-\lambda) n} \cost{J}{J} 
%  \end{align*}
% \end{proof}

\begin{lemma}
\label{lemma:I}
Let $z^1_{i,j}$ be the average of $I_{i,j} \cap P_{i,j},  z^2_{i,j}$ the average of $I_{i,j} \setminus P_{i,j}$, then
\begin{align*}
    |z^1_{i,j}  - \overline{I_{i,j}} | \leq \frac{\err \diam{I_{i,j}}}{1-\err -\bb}
\end{align*}
\end{lemma}
\begin{proof}
We know $|I_{i,j} \cap P_{i,j}| \geq (1-\err -\bb - q) m_i, |I_{i,j} \setminus P_{i,j}| \leq q m_i$ for $q \leq \alpha$. We have 
\begin{align*}
    &\overline{I_{i,j}} = \frac{(1-\err -\bb - q)  z^1_{i,j} + q z^2_{i,j}}{1-\err -\bb} \\ 
    & \implies |z^1_{i,j}  - \overline{I_{i,j}} |  \leq  \frac{q |z^1_{i,j} - z^2_{i,j}|}{1-\err -\bb} \leq  \frac{\err\diam{I_{i,j}}}{1-\err -\bb}
\end{align*}
\end{proof}

% \begin{lemma}
% For all $i \in [k], j \in [d]$, $|\overline{I_{i,j}} - \overline{X^\star_{i,j}}|^2 \leq 3 \left(  \frac{\err \cost{X_{i,j}^\star}{X_{i,j}^\star}}{(1-\err) m_i^\star} + \frac{(\err + \bb) \cost{X_{i,j}^\star}{X_{i,j}^\star} }{(1-2\err - \bb)(1-\err) m_i^\star} + \frac{4\err^2 \cost{X_{i,j}^\star}{X_{i,j}^\star}}{\beta (1-\err) m_i^\star}  \right) $
% \end{lemma}
% \begin{proof}
% By \cref{lemma:lambda_mean}, we have
% \begin{align*}
%     |\overline{P_{i,j}} - X_{i,j}^\star|^2 \leq \frac{\err \cost{X_{i,j}^\star}{X_{i,j}^\star}}{(1-\err) m_i^\star}
% \end{align*}
%  Note that 
% \begin{align*}
%     |I_{i,j} \cap  P_{i,j}| \geq m_i(1-\err - \bb) - \err m_i \geq  |P_i| - m_i(\err + \bb) = |P_i| \left(1 - \frac{ m_i(\err + \bb) }{|P_i|} \right) \geq |P_i| \left(1 - \frac{\err + \bb }{1-\err} \right)
% \end{align*}

% We also have $|P_{i,j} \setminus I_{i,j}| \leq |P_i| \left(\frac{\err + \bb }{1-\err} \right)$. By \cref{lemma:lambda_mean} \begin{align*}
%     |z_{i,j} - \overline{P_{i,j}} |^2 \leq \frac{(\err + \bb) \cost{P_{i,j}}{P_{i,j}}}{(1-2\err - \bb) |P_i|} \leq  \frac{(\err + \bb) \cost{X_{i,j}^\star}{X_{i,j}^\star} }{(1-2\err - \bb)(1-\err) m_i^\star}
% \end{align*}

% We also have 
% \begin{align*}
%     |z_{i,j} - \overline{I_{i,j}}|^2 \leq \err^2 \diam{I_{i,j}} ^2 \leq \frac{4\err^2 \cost{X_{i,j}^\star}{X_{i,j}^\star}}{\beta m_i} \leq \frac{4\err^2 \cost{X_{i,j}^\star}{X_{i,j}^\star}}{\beta (1-\err) m_i^\star} 
% \end{align*}
% Finally,

% \begin{align*}
%     |\overline{I_{i,j}} - \overline{X_{i,j}^\star} |^2 \leq 3 \left(  \frac{\err \cost{X_{i,j}^\star}{X_{i,j}^\star}}{(1-\err) m_i^\star} + \frac{(\err + \bb) \cost{X_{i,j}^\star}{X_{i,j}^\star} }{(1-2\err - \bb)(1-\err) m_i^\star} + \frac{4\err^2 \cost{X_{i,j}^\star}{X_{i,j}^\star}}{\beta (1-\err) m_i^\star}  \right)
% \end{align*}

% \end{proof}

\begin{lemma}
\label{lemma:dist2}
Suppose $2\err + \bb  \in (0, 1]$, we have for all $i \in [k], j \in [d]$,
\begin{align*}
    |\overline{I_{i,j}} - \overline{X^\star_{i,j}}|^2 \leq   \frac{ (4\err + 2\bb) \cost{X_{i,j}^\star}{X_{i,j}^\star} }{(1-2\err - \bb) m_i^\star }   +\frac{8\err^2 \cost{X_{i,j}^\star}{X_{i,j}^\star}}{\beta (1-\err) (1-\err - \bb)^2   m^\star_i} .
\end{align*}
\end{lemma}
\begin{proof}
We know 
\begin{align*}
 |I_{i,j} \cap  X_{i,j}^\star|  =       |I_{i,j} \cap  P_{i,j}| \geq m_i(1-\err - \bb) - \err m_i & \geq  |P_i| - m_i(\err + \bb) \\ & = |P_i| \left(1 - \frac{ m_i(\err + \bb) }{|P_i|} \right) \\ & \geq |P_i| \left(1 - \frac{\err + \bb }{1-\err} \right) \\  & \geq  (1-\err) m_i^\star \left(1 - \frac{\err + \bb }{1-\err} \right) \\ &  = m_i^\star \left(1 - 2\err - \bb \right),
\end{align*}
where we use the fact that $|P_i| \geq (1-\err) m_i^\star $. We can then apply \cref{lemma:lambda_mean} since  $2\err + \bb  \in (0,1]$,
\begin{align*}
    |z_{i,j} - \overline{X_{i,j}^\star}|^2 \leq   \frac{ (2\err + \bb) \cost{X_{i,j}^\star}{X_{i,j}^\star} }{(1-2\err - \bb) m_i^\star } 
\end{align*}
From \cref{lemma:I}, we also have 
\begin{align*}
    |z_{i,j} - \overline{I_{i,j}}|^2 \leq \frac{\err^2 \diam{I_{i,j}} ^2}{(1-\err - \bb)^2} \leq \frac{4\err^2 \cost{X_{i,j}^\star}{X_{i,j}^\star}}{\beta (1-\err - \bb)^2   m_i} \leq \frac{4\err^2 \cost{X_{i,j}^\star}{X_{i,j}^\star}}{\beta (1-\err) (1-\err - \bb)^2   m^\star_i} %\leq \frac{4\err \cost{X_{i,j}^\star}{X_{i,j}^\star}}{ \bb (1-\err) m_i^\star} 
\end{align*} 
Thus we have, 
\begin{align*}
    |\overline{I_{i,j}} - \overline{X_{i,j}^\star} |^2 \leq 2 \left(   \frac{ (2\err + \bb) \cost{X_{i,j}^\star}{X_{i,j}^\star} }{(1-2\err - \bb) m_i^\star }   +\frac{4\err^2 \cost{X_{i,j}^\star}{X_{i,j}^\star}}{\beta (1-\err) (1-\err - \bb)^2   m^\star_i}     \right)
    \end{align*}
    
\end{proof}

\begin{lemma}
Suppose $\err \in (0, 1/7]$ and $\bb = \alpha$, for all $i \in [k], j \in [d]$, $\cost{X^\star_{i,j}}{I_{i,j}} \leq (1 + 29\err) \cost{X^\star_{i,j}}{X^\star_{i,j}}  $
\end{lemma}
\begin{proof}
From \cref{lemma:dist2}, we have 
\begin{align*}
    |\overline{I_{i,j}} - \overline{X_{i,j}^\star} |^2 \leq  \frac{6\err  \cost{X_{i,j}^\star}{X_{i,j}^\star} }{(1-3\err) m_i^\star }   + \frac{8\err \cost{X_{i,j}^\star}{X_{i,j}^\star}}{(1-\err) (1-2\err)^2   m^\star_i}   \leq  \frac{29 \alpha \cost{X_{i,j}^\star}{X_{i,j} }}{ m_i^\star}
    \end{align*}

We thus know, 
\begin{align*}
   & \cost{X^\star_{i,j}}{I_{i,j}}  = \cost{X^\star_{i,j}}{X^\star_{i,j}} + m^\star_i | X^\star_{i,j} -  \overline{I_{i,j}}|^2 \leq (1 + 29\err) \cost{X^\star_{i,j}}{X^\star_{i,j}}
\end{align*}.


\end{proof}

Suppose $I_{i,j}$ is the subset of $X_{i,j}$ of cardinality $(1-\alpha)|X_{i,j}|$ with the minimum cost.
\begin{lemma}
\label{lemma:interval}
\[
|\overline{I_{i,j}} - \overline{P_{i,j}}|^2 \le \frac{4\alpha}{1-2\alpha}\frac{\cost{P_{i,j}}{P_{i,j}}}{|P_{i,j}|}
\]
\end{lemma}
\begin{proof}
By definition, $\cost{I_{i,j}}{I_{i,j}}\le \frac{(1-\alpha) m_i}{|P_{i,j}|}\cost{P_{i,j}}{P_{i,j}}$ (the RHS can be obtained by taking a random subset of $P_{i,j}$ of size exactly $(1-\alpha)m_i$).
Thus, by \cref{lemma:lambda_mean},
\begin{align*}
|\overline{I_{i,j}} - \overline{I_{i,j}\cap P_{i,j}}|^2&\le \frac{|X_{i,j}\setminus P_{i,j}| \cost{I_{i,j}}{I_{i,j}}}{((1-\alpha)m_i-|X_{i,j}\setminus P_{i,j}|)(1-\alpha)m_i} \\  & \leq \frac{|X_{i,j}\setminus P_{i,j}| \cost{P_{i,j}}{P_{i,j}} }{((1-\alpha)m_i-|X_{i,j}\setminus P_{i,j}|) |P_{i,j}|}  \\ & \leq  \frac{\alpha m_i \cost{P_{i,j}}{P_{i,j}}}{(|P_{i,j}|-\alpha m_i)|P_{i,j}|} \\ & =  \frac{\alpha  \cost{P_{i,j}}{P_{i,j}}}{(1-2\alpha)|P_{i,j}|}
% |\overline{P_{i,j}} - \overline{I_{i,j}\cap P_{i,j}}|^2&\le \frac{\alpha m_i \cost{P_{i,j}}{P_{i,j}}}{(|P_{i,j}|-\alpha m_i)|P_{i,j}|}
\end{align*}
, where we use the fact that $|X_{i,j}\setminus P_{i,j}| \leq \err m_i$. 
Also, by \cref{lemma:lambda_mean}, 
\begin{align*}
    |\overline{P_{i,j}} - \overline{I_{i,j}\cap P_{i,j}}|^2&\le \frac{\alpha m_i \cost{P_{i,j}}{P_{i,j}}}{(|P_{i,j}|-\alpha m_i)|P_{i,j}|} \le  \frac{\alpha  \cost{P_{i,j}}{P_{i,j}}}{(1-2\alpha m_i)|P_{i,j}|}
\end{align*}
We conclude the proof by noting that 
\begin{align*}
    |\overline{I_{i,j}} - \overline{P_{i,j}}|^2 \le 2 |\overline{I_{i,j}} - \overline{I_{i,j}\cap P_{i,j}}|^2 + 2 |\overline{I_{i,j}\cap P_{i,j}} - \overline{P_{i,j}}|^2.
\end{align*}
\end{proof}



\begin{lemma}
\[
|\overline{X^\star_{i,j}} - \overline{I_{i,j}}|^2 \le \cost{X^\star_{i,j}}{X^\star_{i,j}} \left(\frac{\alpha}{1-\alpha} + \frac{4\alpha}{(1-2\alpha)(1-\alpha)}\right)/m^\star_i
\]
\end{lemma}
\begin{proof}
 By \cref{distJ_J2},
\begin{align*}
% &|\overline{X^\star_{i,j}} - \overline{P_{i,j}}|^2 = z^2 |\overline{X^\star_{i,j}\setminus P_{i,j}} - \overline{P_{i,j}}|^2 \\
&|\overline{X^\star_{i,j}} - \overline{X^\star_{i,j} \setminus P_{i,j}}|^2 = \frac{(1-z)^2}{z^2} |\overline{X^\star_{i,j}} - \overline{P_{i,j}}|^2 , 
\end{align*}
where $z = \frac{|X^\star_{i,j}\setminus P_{i,j}|}{|X^\star_{i,j}|}\le \alpha$. We have
\begin{align*}
    & \cost{X^\star_{i,j}}{X^\star_{i,j}} \\ &= \cost{X^\star_{i,j} \setminus P_{i,j}}{X^\star_{i,j}}  + \cost{P_{i,j}}{X^\star_{i,j}}  \\ &= \cost{X^\star_{i,j} \setminus P_{i,j}}{X^\star_{i,j} \setminus P_{i,j}} + z m^\star_i |\overline{X^\star_{i,j}} - \overline{X^\star_{i,j} \setminus P_{i,j}}|^2  + \cost{P_{i,j}}{P_{i,j}} + (1-z)m^\star_i |\overline{X^\star_{i,j}} - \overline{P_{i,j}}|^2  \\ & =  \frac{1-z}{z} m^\star_i|\overline{X^\star_{i,j}} - \overline{P_{i,j}}|^2   + \cost{X^\star_{i,j} \setminus P_{i,j}}{X^\star_{i,j} \setminus P_{i,j}}   +  \cost{P_{i,j}}{P_{i,j}} \\
    & \geq \frac{1-\err}{\err} m^\star_i|\overline{X^\star_{i,j}} - \overline{P_{i,j}}|^2  +  \cost{P_{i,j}}{P_{i,j}}. 
\end{align*}

Applying \cref{lemma:interval}, we have 
\[
\cost{X^\star_{i,j}}{X^\star_{i,j}} \ge \frac{1-\alpha}{\alpha} m^\star_i|\overline{X^\star_{i,j}} - \overline{P_{i,j}}|^2 + \frac{1-2\alpha}{4\alpha}\cdot (1-\alpha)m^\star_i |\overline{I_{i,j}} - \overline{P_{i,j}}|^2.
\]
By Cauchy-Schwarz,
\begin{align*}
   & \left(|\overline{X^\star_{i,j}} - \overline{P_{i,j}}|+|\overline{I_{i,j}} - \overline{P_{i,j}}|\right)^2 \\ & \le \left(\frac{\alpha}{1-\alpha} + \frac{4\alpha}{(1-2\alpha)(1-\alpha)}\right) \left(  \frac{1-\alpha}{\alpha}   m^\star_i|\overline{X^\star_{i,j}} - \overline{P_{i,j}}|^2 + \frac{1-2\alpha}{4\alpha}\cdot (1-\alpha)m^\star_i |\overline{I_{i,j}} - \overline{P_{i,j}}|^2 \right)/m^\star_i  \\ & \le \cost{X^\star_{i,j}}{X^\star_{i,j}} \left(\frac{\alpha}{1-\alpha} + \frac{4\alpha}{(1-2\alpha)(1-\alpha)}\right)/m^\star_i
\end{align*}
We conclude the proof by the fact that $|\overline{X^\star_{i,j}} - \overline{I_{i,j}}|^2 \leq \left(|\overline{X^\star_{i,j}} - \overline{P_{i,j}}|+|\overline{I_{i,j}} - \overline{P_{i,j}}|\right)^2 $.

\end{proof}

==> prelims.tex <==
\section{Preliminaries}

\newcommand{\dist}{\mathrm{dist}}

We start by formally restating the problem at hand.

\begin{definition}[Learning augmented clustering]
    \begin{enumerate}
        \item We are given a data set $P \subset \R^d$, $m:= |P|$. The ambient space of the data set is equipped with some distance function $\dist (\cdot, \cdot)$ which is a metric. We denote the \emph{cost} of the data set $P$ with respect to a set $C$ by $\costP(P,C)$, and this cost is defined by the expression
        \begin{align*}
            \costP{P}{C} = \sum_{p\in P} \min_{c\in C} \dist (p,c).
        \end{align*}
        \item We let $\OPT$ denote the optimally low clustering cost of $P$ with respect to sets $C$ of size $k$, i.e. $\OPT = \min_{C:|C|\leq k} \costP{P}{C}$.
        \item We are also given an expert labelling $P_1, \dots, P_k$ which is a partition of $P$ and a label error rate $\alpha \in [0,1)$ with the promise that there exists some optimal clustering $P_1^*, \dots, P_k^*$ and corresponding cluster centers $C^* = \{c_1^*, \dots c_k^*\}$ such that $\costP{P}{C^*} = \OPT$, and such that $|P_i\cap P_i^*| \geq (1-\alpha)\max(|P_i|, |P_i^*|)$.
    \end{enumerate}
    
    We now recall some results from prior work which we will appeal to in the sequel.
     
\end{definition}
